Assessing the Performance of Leja and Clenshaw-Curtis Collocation for Computational Electromagnetics with Random Input Data

We consider the problem of quantifying uncertainty regarding the output of an electromagnetic field problem in the presence of a large number of uncertain input parameters. In order to reduce the growth in complexity with the number of dimensions, we employ a dimension-adaptive stochastic collocation method based on nested univariate nodes. We examine the accuracy and performance of collocation schemes based on Clenshaw-Curtis and Leja rules, for the cases of uniform and bounded, non-uniform random inputs, respectively. Based on numerical experiments with an academic electromagnetic field model, we compare the two rules in both the univariate and multivariate case and for both quadrature and interpolation purposes. Results for a real-world electromagnetic field application featuring high-dimensional input uncertainty are also presented.

==> images/Geometry.tex <==
\pgfplotsset{
tick label style={font=\footnotesize},
label style={font=\footnotesize},
legend style={font=\footnotesize}
}

\begin{tikzpicture}

\begin{axis}[
width=\columnwidth,
height=0.65\columnwidth,
cycle list name=color list,
xtick={-8,-6,-4,-2,0,2,4,6,8},
xticklabels={-8,-6,-4,-2,0,2,4,6,8},	
xlabel={\footnotesize x / mm},
xlabel near ticks,
xmin=-8,
xmax=5,
ytick={0,1,2,3,4,5,6,7,8,9,10,15,20},	
yticklabels={0,1,2,3,4,5,6,7,8,9,10,15,20},	
ylabel={\footnotesize y / mm},
%ylabel style={yshift=-0.4cm},
ylabel near ticks,
ymin=0,
ymax=8,
%legend style={legend columns=-1},
legend style={at={(0.02,0.98)},anchor=north west},
legend entries={Original geometry, Original control points,Optimized geometry},
]

\addplot[blue,thick, dashed] table[x index=0, y index=1] {Data/OriginalConcave.dat};
\addplot[blue,thick, dashed, forget plot] table[x index=0, y index=1] {Data/OriginalConvex.dat};
\addplot[mark=*, mark size=1.5pt, only marks, blue, forget plot] table[x index=0, y index=1] {Data/convexCtrlPoints.dat};
\addplot[mark=*, mark size=1.5pt, only marks, blue] table[x index=0, y index=1] {Data/concaveCtrlPoints.dat};
\addplot[red,thick] table[x index=0, y index=1] {Data/OptimConcave.dat};
\addplot[red,thick, forget plot] table[x index=0, y index=1] {Data/OptimConvex.dat};
%\addplot[thick] table[x index=0, y index=1] {Data/BeamArea.dat};
\draw [fill=gray, gray] (axis cs:-1.5,0) rectangle (axis cs:-1.0,3);

\node at (axis cs:-2,2) [anchor=south] {1};
\node at (axis cs:-4,4) [anchor=south west] {2};
\node at (axis cs:2,2) [anchor=south west] {3};
\node at (axis cs:-0.5,4.5) [anchor=south west] {4};
\node at (axis cs:-2,0) [anchor=south east] {1'};
\node at (axis cs:2,0) [anchor=south east] {3'};


\end{axis}

\end{tikzpicture}
